Grid-Aware Islanding and Resynchronisation of AC/DC Microgrids

This paper proposes an optimal, grid-aware control framework for the islanding, island-operation and resynchronisation of hybrid AC/DC microgrids. The optimal control framework is based on a formally derived linearized load-flow model for multiterminal hybrid AC/DC networks. The load flow model integrates the AC grid, DC grid, and interfacing converters (IC) into a unified representation. This work extends an existing load flow model to include the ICs' grid-forming operation. In traditional islanding control frameworks, the grid-forming converter is typically interfaced with an energy storage system that can provide bidirectional power to maintain the power balance. The proposed framework, however, allows the ICs to operate as the grid-forming unit while being connected to a DC grid rather than a single resource. This configuration allows for a wider operating range and, thus, a more flexible control. Furthermore, the optimal grid-aware control framework can steer the system to ensure a feasible operation without any grid constraint violations before, during, and after the islanding manoeuvre. The framework also guarantees smooth transitions, i.e., without any significant transient behaviour, when transitioning between grid-connected and islanding operations. The optimal control framework is experimentally validated on a 27-bus hybrid AC/DC network consisting of 3 ICs that interface the AC and DC networks. The hybrid grid hosts various controllable and stochastic resources.

==> sections/Stateoftheart.tex <==
\section{State-of-the-art review} 
\label{sec:stateoftheart}

Everything done so far is droop control, no central

some optimal grid aware control of solely AC grid. No DC grid. But as discussed in the introduction, the problem formulation is fundamentally different because the power required to maintain the AC voltage setpoints are provided by an energy supply




